Minimum Enclosing Parallelogram with Outliers

We study the problem of minimum enclosing rectangle with outliers, which asks to find, for a given set of $n$ planar points, a rectangle with minimum area that encloses at least $(n-t)$ points. The uncovered points are regarded as outliers. We present an exact algorithm with $O(kt^3+ktn+n^2\log n)$ runtime, assuming that no three points lie on the same line. Here $k$ denotes the number of points on the first $(t+1)$ convex layers. We further propose a sampling algorithm with runtime $O(n+\mbox{poly}(\log{n}, t, 1/\epsilon))$, which with high probability finds a rectangle covering at least $(1-\epsilon)(n-t)$ points with at most the exact optimal area.

==> adaption.tex <==
%!TeX root = main.tex
\section{Smallest Enclosing Rectangle of Arbitrary Orientation}
\label{sec:adaption}
In this part, we illustrate how the techniques developed so far in this work can be adapted to the \MER\ of arbitrary orientation. For the exact solution, we can improve the time complexity $O(n^{2}t^{2}+n^{2}t\log{n})$ given in \cite{das2005smallest} to $O(n^{2}t^{2}+n^{2}\log{n})$. For the approximate solution, we can apply Lemma~\ref{sampling} and further reduce the time complexity when $n$ is large.

\subsection{Exact Solution}
To adopt our algorithm to \MER, we first need the following observation.

\begin{lemma}[{\cite[Theorem 2.1]{toussaint1983solving}}]
The rectangle of minimum area enclosing a convex polygon has a side collinear with one of the edges of the polygon.
\end{lemma}

Let $P_{1}$, $P_{2}$ denote the two points on the collinear side, $P_{3}$ denote the one on the parallel side, and $Q_{1}$, $Q_{2}$ denote the point on the other two sides of the rectangle, respectively. Similar to our discussion in Section~\ref{sec:timealg}, $(P_{1}, P_{2})$ must be a valid pair and there are $O(nt)$ of them. Given $P_{1}$ and $P_{2}$, the point $P_{3}$ must be among the $(t+2)$ farthest points on the majority side from the line $P_{1}P_{2}$. At the same time, $Q_{1}$ and $Q_{2}$ must be among the leftmost and rightmost $(t+2)$ points along the direction of the line $P_{1}P_{2}$. And it takes time $O(nt)$ to find all the candidates for $P_{3}$, $Q_{1}$ and $Q_{2}$. Furthermore, with given $Q_{1}$ and $Q_{2}$, there is at most one possible $P_{3}$ and we can find it in $O(1)$ time. Therefore there are $O(t^{2})$ combinations of $Q_{1}$, $Q_{2}$ and $P_{3}$. We finally enumerate over all the combinations of $P_{1}$, $P_{2}$, $P_{3}$, $Q_{1}$ and $Q_{2}$ and select the one whose determined rectangle has smallest area.

As regards the time complexity of the algorithm above, we have
\begin{theorem}
	\label{thm:main1} 
	Given a set $\bX$ of $n$ planar points, the optimal solution $sol^\ast_{\MEP,t}(\bX)$ can be found in $O(k^{2}t^{4}+n^{2}\log{n})$ time and $O(kt^2)$ space.
\end{theorem}

\begin{proof}
First of all, it takes time $O(nt)$ to find all the candidates of $P_{3}$, $Q_{1}$ and $Q_{2}$ when $P_{1}$ and $P_{2}$ are given. As there are $O(nt)$ valid pairs $(P_{1}, P_{2})$, the time complexity to find all the valid pairs and all the candidates of $P_{3}$, $Q_{1}$ and $Q_{2}$ is $O(n^{2}\log{n}+n^{2}t^{2})$. On the other hand, there are $O(nt)\times O(t^{2})=O(nt^{3})$ valid combinations of $P_{1}$, $P_{2}$, $P_{3}$, $Q_{1}$ and $Q_{2}$. Simply enumerating over all the combinations and computing the area of the rectangle determined by each of the combinations takes time $O(nt^{3})$. The time complexity of the algorithm is $O(n^{2}\log{n}+n^{2}t^{2}+nt^{3})=O(n^{2}\log{n}+n^{2}t^{2})$.
\end{proof}

\subsection{Approximate Solution}
In a similar manner as Lemma~\ref{VC dimension}, we can prove that the VC dimension of the rectangles is also at most 9. Then the same statements and arguments in Section~\ref{sec:approximation} can be applied to the \MER\ of arbitrary orientation. Sampling $s=O\left(\frac{\log{n}}{\epsilon^{2}}\right)$ from $n$ points takes $O(n)$ time, and the number of outliers in the $s$ sampled points becomes $t^{\prime}=O\left(\left(\frac{t}{n}+\epsilon\right)s\right)$. By replacing $n$ by $s$, $t$ by $t^{\prime}$ in $O(n^{2}\log{n}+n^{2}t^{2})$, and adding the sampling time $O(n)$, we obtain the time complexity of the approximation algorithm $O\left(n+\left(\frac{\log{n}}{\epsilon^{2}}\right)^{4}\left(\frac{t}{n}+\epsilon\right)^2\right)$.

==> previouswork.tex <==
%!TeX root = main.tex
\subsection{Related Works}
A lot of research in computational geometry concerns finding a shape which encloses a given Euclidean point set. They are known as shape fitting problems \cite{har2004shape} and have been widely studied in different communities such as computational geometry, computer graphics and data mining. Many problems can be classified into this category, including the convex hull, convex layers, minimum enclosing parallelogram, smallest enclosing rectangle, $k$-means/median clustering and Gaussian mixture model. We now review the most relevant ones below, with and without outliers.

Given a planar point set of size $n$, the famous Quickhull algorithm~\cite{barber1996quickhull} finds the convex hull with average case complexity $O(n\log{n})$ and worst case complexity $O(n^{2})$. Many optimal algorithms have been developed for different dimension $d$. For $d=2$, the Kirkpatrick-Seidel algorithm~\cite{kirkpatrick1986ultimate} achieves the optimal worst case time complexity $O(n\log{N})$, where $N\leq n$ is the convex hull size and in general much smaller than $n$. The first optimal algorithm for $d=3$ is given in~\cite{chazelle1995derandomizing}, and the time complexity is also $O(n\log{N})$. Furthermore, another optimal algorithm for $d=2$ is given in \cite{chan1996optimal}, and its extension to $d=3$ also achieves the optimal time complexity $O(n\log{N})$. When $d>3$, an algorithm with optimal complexity $O(n^{\lfloor d/2\rfloor})$ is given in~\cite{chazelle1993optimal}. 

Convex layers are a natural extension of the convex hull. The convex layers of a point set are a sequence of nested convex polygons, where the $(t+1)$-st layer is defined to be the convex hull of the remaining points after those on the first $t$ layers are removed. An important application is to robust statistic \cite{eddy1982convex}, where the points on the first few layers are identified as outliers, hoping to improve the measurement of the central tendency of the point set by removing these outliers in advance. An optimal algorithm to find all the convex layers with runtime $O(n\log{n})$ is presented in \cite{chazelle1985convex}.

Another variant of the problem, which also involves outliers, is defined in~\cite{atanassov2006removing}. Here the task is to find a convex polygon with smallest area that encloses at least $(n-t)$ points, and the other points are recognized as outliers. An exact algorithm with time complexity $O(n\log{n}+n(3t)^{t}{4t\choose{2t}})$ is given in~\cite{atanassov2006removing}. As the resulting convex polygon is simply the convex hull of the enclosed points, and there are at most $t$ points being excluded outside the polygon, the problem is known as the convex hull with outliers.

Closely related to the convex hull problem are the smallest enclosing square (SES), smallest enclosing rectangle (SER) and the minimum enclosing parallelogram (MEP). Allowing to exclude $t<n/2$ points as outliers, there were $O(n+t^2n)$ time algorithms for both SES~\cite{smid1993finding} and SER~\cite{segal1998enclosing}, both under the assumption that the square/rectangle has to be axis-parallel. The runtimes were later improved to $O(n+t\log^{2}{t})$ for SES and, when $t < n/\log^2 n$, to $O(n+t^3\log^{2}{n})$ for SER~\cite{mahapatra2011k}. Removing the axis-parallel constraint is more complicated. Finding the SER with arbitrary orientation leads to a significantly higher runtime of $O(n^{2}t^{2}+n^{2}t \log{n})$ for $t<n/2$~\cite{das2005smallest}, which has been recently improved to 
$O(n\log^{2}{n}+(n-t)^{2}n\log{n})$ for large $t = \Omega(\sqrt{n\log n})$~\cite{de2016covering}.

Regarding the MEP, an $O(N)$ algorithm is known to find the MEP of a given convex polygon with $N$ vertices~\cite{schwarz1994finding}.  Together with the algorithms in \cite{kirkpatrick1986ultimate} or \cite{chan1996optimal}, we can find the MEP of $n$ planar points in $O(n\log N)$ time by finding the convex hull first in $O(n\log N)$ time. The MEP of the convex hull is also an MEP of the points. Instead of enclosing the whole point set with a parallelogram of smallest area as in \cite{schwarz1994finding}, in this work we take outliers into consideration. We also generalize the techniques to rectangles of arbitrary orientation in the outlier case in Section~\ref{sec:adaption}.

